A General Framework for Multi-fidelity Bayesian Optimization with Gaussian Processes

How can we efficiently gather information to optimize an unknown function, when presented with multiple, mutually dependent information sources with different costs? For example, when optimizing a robotic system, intelligently trading off computer simulations and real robot testings can lead to significant savings. Existing methods, such as multi-fidelity GP-UCB or Entropy Search-based approaches, either make simplistic assumptions on the interaction among different fidelities or use simple heuristics that lack theoretical guarantees. In this paper, we study multi-fidelity Bayesian optimization with complex structural dependencies among multiple outputs, and propose MF-MI-Greedy, a principled algorithmic framework for addressing this problem. In particular, we model different fidelities using additive Gaussian processes based on shared latent structures with the target function. Then we use cost-sensitive mutual information gain for efficient Bayesian global optimization. We propose a simple notion of regret which incorporates the cost of different fidelities, and prove that MF-MI-Greedy achieves low regret. We demonstrate the strong empirical performance of our algorithm on both synthetic and real-world datasets.

==> notes-main.tex <==
\include{macros}

% add line numbers for drafting
% comment these sections out in submissions
% \linenumbers
\nocopyright

\begin{document}
% The file aaai.sty is the style file for AAAI Press
% proceedings, working notes, and technical reports.
%
% \title{Multi-fidelity Bayesian Optimization via Gaussian Processes: \\Theory and Applications}
% \title{Cost-effective Bayesian Optimization with Multi-fidelity Gaussian Process}
% \title{Multi-fidelity Max-value Entropy Search with Convolved Gaussian Process}
\title{Multi-fidelity Bayesian Optimization with Convolved Gaussian Process}

\author{
  Anonymous Authors\\
  % Paper ID \#
  % Jialin Song\\ Caltech\\ jssong@caltech.edu
  % \And
  % Yuxin Chen \\ Caltech \\ chenyux@caltech.edu
  % \And
  % Yisong Yue \\ Caltech \\ yyue@caltech.edu
}
% \maketitle

% % ---------- abstract ------------
% \input{abstract}
% % ---------- introduction ------------
% \input{intro}
% % ---------- related ------------
% \input{related}
% % ---------- problem statement ------------
% \input{statement}
% % ---------- method ------------
% \input{method}
% % ---------- analysis ------------
% \input{analysis}
% % ---------- experiments ------------
% \input{exp}
% % ---------- conclusion ------------
% \input{conclusion}
% % % ---------- acknowledgment ------------
% % \input{ack}


\input{notes}

% \clearpage
% \nolinenumbers
% \bibliography{reference}
% \bibliographystyle{aaai}

% % ---------- appendices ------------
% \appendix
% \input{appendix}

\end{document}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> notes.tex <==
% !TEX root = ./notes-main.tex

% \vspace{3cm}
% \paragraph{NOTES}
% \begin{itemize}\denselist
% \item By submodularity of the mutual information, we know that the maximal information gain of \sfgpopt under budget $\budget-\epcost$ conditioning on having performed actions $\epselected$, is no larger than the maximal information gain.
% \end{itemize}


\section{Problem Statement}
In this sections, we define necessary notations, and formally state the problem studied in this paper.
\subsection{Preliminary on Gaussian Processes}
Notations\\
\begin{itemize}\denselist
\item Fidelity indices: $1, \dots, i, \dots, \targetfid$; index of the target fc $\targetfid$
\item Cost of $i$-th fidelity $\costof{i}$
\item target fidelity function: $\tarf$
\item Budget $\budget$
\end{itemize}
..\\
..\\
..\\
..\\
..\\
\subsection{Regret for multi-fidelity bandit optimization}
\begin{definition} % An \emph{episode} is a sequence of actions, where the last action is from the target fidelity, and all remaining actions are from the lower fidelities.
  Let $n\in \integers$ be any integer. We call a sequence of items $\ep = \{\langle \ex_1, i_1 \rangle, \dots, \langle \ex_n, i_n \rangle\}$ an \emph{episode}, if $\forall \ell < n:\ i_\ell < t$ and $i_n = t$.
\end{definition}
In words, only the last item of an episode is from the target fidelity and all remaining items are from lower fidelities. We now define a simple notion of regret for an episode.
% starts with actions from any fidelity, and terminates at the first occurrence of an action from the target fidelity.
\begin{definition}[Regret]
  % Regret in terms of the cost
  The regret of an episode $\ep = \{\langle x_1, i_1 \rangle, \dots, \langle x_{-1}, t \rangle\}$ is
  \begin{align}
    \regret(\ep) = \frac{\costof{\ep}}{\costof{\targetfid}} \tarf^* - \utility(\ep)
  \end{align}
  where $\costof{\ep} = \sum_{\langle x,i \rangle\in \ep} \costof{i}$ is the total cost of episode $\ep$, and $\utility(\ep) = \tarf\left(x_{-1}\right)$ denotes the function value of the last item on the target fidelity.
\end{definition}

Suppose we run an algorithm $\policy$ under a budget $\budget$ and select a sequence of items. One can divide the sequence of items into multiple episodes $\{\ep_1, \dots, \ep_k\}$; % each ending with an item on the target fidelity.
clearly, $\sum_{j=1}^k \costof{\ep_j} \leq \budget$.
The cumulative regret is defined as
\begin{align}
  % \cumreg = \sum_{j=1}^k \regret(\ep_j)
  \cumreg(\policy) = \frac{\budget}{\costof{\targetfid}} \tarf^* - \sum_{j=1}^k \utility(\ep_j)
\end{align}
Similarly with the single-fidelity case, a desirable asymptotic property of an algorithm is to be \emph{no-regret}.
% Our goal, is to minimize the regret/ achieve low regret.
\\
..\\
..\\
..\\
..\\
..\\
..\\
..\\
..\\
..\\
..\\
\subsection{Algorithm}
Our algorithm is presented in \algref{alg:main}. % \figref{fig:alg:illustration} illustrate \algref{alg:main} in two different iterations.
\setlength{\textfloatsep}{14pt}
\begin{algorithm}[t!]
  \nl {\bf Input}: {Input domain; multi-fidelity oracle; evaluation cost at each fidelity; Prior on latent process and noise}; \\
  % \nl {\bf Output}: {}; \\
  % \nl {\bf Parameters}: {}; \\
  \Begin{
    \nl Initiailize convolved Gaussian processes for each fidelity; \label{algln:ln}\\
    % \ForEach{}{
    % \nl ; \\
    % }
    \While{stopping condition not reached}
    {
      \nl Jointly select fidelity and input using cost-sensitive max-value entropy search
      \nl update convolved GP.
    }
    \nl {\bf Output}: optimizer of the target function \\
  }
  \caption{Multi-fidelity Max-value Entropy Search (\algname)}\label{alg:main}
\end{algorithm}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "notes-main"
%%% End:


==> notes_backup.tex <==
\clearpage
% \begin{lemma}
%   %   Let us set $\beta_1, \dots, \beta_k$ such that
%   %   Then, it holds that the average cumulative regret of \algname
%   Assume $\beta_1\leq \dots \leq \beta_k$, and $\sum_j \beta_j^{-1} = \littleO{\sqrt{\budget}}$. Then, the average cumulative regret of \algname satisfies
%   \begin{align*}
%     \cumreg(\policy,\budget) \leq \sqrt{\constgeneral \budget \paren{\gamma - \gamma_1}} + \gamma_\eplow(\beta_1) \cdot \littleO{\sqrt{\budget}}
%   \end{align*}
%   where $\gamma_1$ is the mutual information obtained by the lower fidelity actions within the first episode when running \algname, and $\gamma_\eplow(\beta_1)$ is the mutual information obtained by running the greedy benefit-cost-ratio algorithm until the cumulative benefit-cost ratio goes below $\beta_1$.
% \end{lemma}
\begin{proof}
  Suppose we run the benefit-cost ratio greedy algorithm on low fidelities until the cumulative benefit-cost ratio goes below $\beta_1$. Denote the set of actions selected by such algorithm as $\eplow$. We thus have
  \begin{align*}
    &\frac{\infgain{\bobs_{\eplow}}}{\eplowcost } \geq \beta_1 \\
    \forall \action{\ex, \fid}:\  &\frac{\infgain{\bobs_{\eplow} \cup \{\action{\ex, \fid}\}}}{\eplowcost + \costof{\fid}} < \beta_1
  \end{align*}
  Let $\gamma_\eplow(\beta_1) := \infgain{\bobs_{\eplow}}$ be the mutual information gathered by such algorithm. Is is easy to show that $\forall j\geq 1$,
  \begin{align}
    \label{eq:1}
    \gamma_\eplow(\beta_1)
    &= \infgain{\bobs_{\eplow}} \nonumber \\
    &\stackrel{\textcolor{red}{?}}{\geq} \condinfgain{\bobs_{\eplow}^{(j)} }{\bobs_{\epselected}^{(1:j-1)}}
  \end{align}
  due to sumbodularity of mutual information, and $\beta_1 \geq \beta_j$. \yuxin{Does the above inequality hold? -- no. We need a separate lemma}

  % \explorelf at the beginning of the session, until
  From Eq~\eqref{eq:app:sumeplowcostbound} we know
  \begin{align*}
    \sum_{j=1}^k{\eplowcostat{j}}
    &\leq \sum_{j=1}^k\frac{\condinfgain{\bobs_{\eplow}^{(j)} }{\bobs_{\epselected}^{(1:j-1)}}}{\beta_j} \\
    &\leq \sum_{j=1}^k\frac{\gamma_\eplow(\beta_1)}{\beta_j} \\
    &= \gamma_\eplow(\beta_1) \cdot \littleO{\sqrt{\budget}}
    % &= \littleO{\sqrt{\budget}} \sum_{j=1}^k \frac{1}{j^2} \condinfgain{\bobs_{\eplow}^{(j)} }{\bobs_{\epselected}^{(1:j-1)}} \\
    % &\leq \littleO{\sqrt{\budget}} \infgain{\bobs_{\eplow}^{(1)} } \sum_{j=1}^k \frac{1}{j^2}
    % &= \frac{\gamma_L}{\beta_1}
  \end{align*}
\end{proof}

TODO:
\yuxin{If we only consider the low-fidelity actions. Does the greedy benefit-cost-ratio algorithm give a near-optimal solution to the following problem?}
\begin{align}
  \label{eq:2}
  \eplow^* = \argmax_{\eplow: \frac{\infgain{\bobs_{\eplow}}}{\eplowcost } \geq \beta_1}  \infgain{\bobs_{\eplow}}
\end{align}


% \begin{lemma}
%   %   In the following, we show that the maximum $\eplowcostat{j}$
%   Define function
%   \begin{align*}
%     g(B) = \frac{\max_{\Cost_{\eplow'}\leq B}\infgain{\bobs_{\eplow'}}}{B}.
%   \end{align*}
%   Then, $g$ is monotone decreasing.
% \end{lemma}
% \begin{proof}
%   Easy to show in the unit cost setting ($B\in \integers$).

%   \yuxin{True for non-uniform cost setting? perhaps not..}
%   %   We want to solve $g(B) = \beta$
% \end{proof}

%


% Next, we show that \algref{alg:main} achieves a regret bound that is no worse than \algref{alg:explore-then-exploit}.
% \begin{lemma}
%   \algref{alg:main} is no worse than \algref{alg:explore-then-exploit}.
% \end{lemma}

% \begin{proof}
%   We consider two different cases.

%   {\bfseries Case 1: $B > UB$ } In this case, it is easy to show that \algref{alg:explore-then-exploit} is no worse that \sfgpopt.

%   todo: need to figure out constants.

%   {\bfseries Case 2: $B < LB$ } When $B$ is very small, \algref{alg:explore-then-exploit} is the same as \sfgpopt (i.e., no exploration).

%   {\bfseries Case 3: $B\in [LB, UB]$} We want to show that when $B$ is in the middle range $[LB, UB]$, \algref{alg:explore-then-exploit} is also performing well.

% \end{proof}
% \begin{proof}[Proof of \thmref{thm:main}]

% \end{proof}


% design an online learning policy to optimize the target fidelity function.

% Different fidelities interact with each other through some unknown joint distribution , which could be learned over time.

% The $\action{\ex, \fid}$ interact with the the payoff function,

% $\Pr(\utility_\fid(\ex) \given \utility_\targetfid)$

% Querying each lower fidelity will reveal some information about the
% We assume that $\utility$ is a sample from the GP distribution, denoted by $\utility\sim \GP{\mean(\ex), \cov(\ex, \ex')}$
% \begin{itemize}\denselist
% \item Fidelity indices: $1, \dots, \fid, \dots, \targetfid$; index of the target fidelity $\targetfid$
% \item Cost of $\fid$-th fidelity $\costof{\fid}$
% \item target fidelity function: $\tarf$
% \item Budget $\budget$
% \end{itemize}



\subsection{Multi-fidelity Convolved Gaussian process}
\begin{figure}[t]
  \centering
  \includegraphics[trim={0pt 0pt 0pt 0pt}, width=.48\textwidth]{./fig/empty.png}
  \includegraphics[trim={0pt 0pt 0pt 0pt}, width=.48\textwidth]{./fig/empty.png}
  \caption{Illustration of GP optimization}
  \label{fig:gp:illustration}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[trim={0pt 0pt 0pt 0pt}, width=.25\textwidth]{./fig/convolved_gp.pdf}
  \caption{Multi-fidelity convolved Gaussian processs}
  \label{fig:conv-gp}
\end{figure}
The $i$-th fidelity $\fidelity_i$ for $i<t$ is defined as the convolution between a latent process $\latentproc_i$ and a smoothing kernel $\convkernel_{ii}$:
\begin{align}
        \fidelity_i(\ex) = \int_{\ex'}\latentproc_i(\ex')\convkernel_{ii}(\ex - \ex')\diff \ex'
      \end{align}
        The target function $\fidelity_t$ is
        \begin{align}
        \fidelity_t(\ex) = \int_{\ex'}\latentproc_i(\ex')\convkernel_{it}(\ex - \ex')\diff \ex'
      \end{align}
        The observed value for fidelity $i\in\{1, \dots, t\}$ is $\obs_i = \fidelity_i + \noise_i$, where $\noise_i$ denotes Gaussian process noise that is independent of $\fidelity_i$.




\begin{algorithm}[t!]
  \nl {\bf Input}: {Budget $\budget$; cost $\costof{i}$ for all fidelities $i \in [\targetfid]$}; joint GP prior on $\{\fidelity_i, \noise_i\}_{i\in[\targetfid]}$\\ % between $\fidelity_i$ and noise $$. \\
  \Begin{
    % \nl $\alpha = \frac{\max_\ex \infgain{\action{\ex, \targetfid}}}{\sqrt{\budget} \costof{\targetfid}} $ \\
    \nl $\selected \leftarrow \emptyset$ \\
    \nl $B \leftarrow \budget$ \tcc*{initialize remainig budget}
    \While{$B > 0$} % outer loop
    {
      \nl $\epselected \leftarrow \emptyset; \Cost_\epselected \leftarrow 0$ \tcc*[r]{initialize an episode}
      \nl $\beta \leftarrow \frac{1}{\littleO{\sqrt{B}}}$ \tcc*{stopping condition}
      % \nl $\Cost_\epselected \leftarrow 0$ \\
      % \nl $\beta \leftarrow \frac{\max_\ex \condinfgain{\obs_{\action{\ex, \targetfid}}}{\bobs_\selected}} {\costof{\targetfid} \sqrt{B}} $ \\
      % \nl $\frac{\condinfgain{\bobs_{\epselected \cup \{ \action{\ex^*, \fid^*} \} }}{\bobs_\selected}}{\paren{\Cost_\epselected + \costof{\fid^*}}} \geq \beta$ \\
      % \While{$\frac{\condinfgain{\bobs_{\epselected \cup \{ \action{\ex^*, \fid^*} \} }}{\bobs_\selected}}{\paren{\Cost_\epselected + \costof{\fid^*}}} \geq \frac{\max_\ex \condinfgain{\obs_{\action{\ex, \targetfid}}}{\bobs_\selected}} {\costof{\targetfid} \sqrt{B}}$} %
      \tcc{explore with lower fidelities}
      \While{true}
      {
        \tcc{greedy benefit-cost ratio}
        \nl $\action{\ex^*, \fid^*} \leftarrow \argmax_{\action{\ex, \fid}} \frac{\condinfgain{\obs_{\action{\ex, \fid}}}{\bobs_{\selected \cup \epselected}}}{\costof{\fid}}$ \\
        % \If{$\fid^*\neq \targetfid$} % stopping condition
        % {
        \If{$\fid^* = \targetfid$ or $\frac{\condinfgain{\bobs_{\epselected \cup \{ \action{\ex^*, \fid^*} \} } }{\bobs_\selected}} {\paren{\Cost_\epselected + \costof{\fid^*}}} < \beta$}
        {
          \tcc{stop an episode}
          \nl break
        }
        \Else
        {
          \nl $\epselected \leftarrow \epselected \cup \{\action{\ex^*,\fid^*}\}$ % \tcc*{explore}
        }
      }
      % \Repeat{$\fid^* = \targetfid$ or $\frac{\condinfgain{\bobs_{\epselected \cup \{ \action{\ex^*, \fid^*} \} } }{\bobs_\selected}} {\paren{\Cost_\epselected + \costof{\fid^*}}} < \beta$}
      % {
      % \nl $\action{\ex^*, \fid^*} \leftarrow \argmax_{\action{\ex, \fid}} \frac{\condinfgain{\obs_{\action{\ex, \fid}}}{\bobs_{\selected \cup \epselected}}}{\costof{\fid}}$ \\
      %   % \If{$\fid^*\neq \targetfid$} % stopping condition
      %   % {
      % \nl $\epselected \leftarrow \epselected \cup \{\action{\ex^*,\fid^*}\}$\\
      %   % }
      % }
      \tcc{select target fidelity}
      \nl $\ex^* \leftarrow \sfgpopt(\GP{\tarf}, \bobs_{\selected \cup \epselected})$ \\
      \nl $\selected \leftarrow \selected \cup \epselected \cup \{\action{\ex^*,\targetfid}\}$\\
      \nl $B \leftarrow \budget - \Cost_\selected$ \tcc*{update remaining budget}
    }
    \nl {\bf Output}: Optimizer of the target function $\tarf$ \\
  }
  \caption{Multi-fidelity GP Optimization}\label{alg:main}
\end{algorithm}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

